On Early-stage Debunking Rumors on Twitter: Leveraging the Wisdom of Weak Learners

Recently a lot of progress has been made in rumor modeling and rumor detection for micro-blogging streams. However, existing automated methods do not perform very well for early rumor detection, which is crucial in many settings, e.g., in crisis situations. One reason for this is that aggregated rumor features such as propagation features, which work well on the long run, are - due to their accumulating characteristic - not very helpful in the early phase of a rumor. In this work, we present an approach for early rumor detection, which leverages Convolutional Neural Networks for learning the hidden representations of individual rumor-related tweets to gain insights on the credibility of each tweets. We then aggregate the predictions from the very beginning of a rumor to obtain the overall event credits (so-called wisdom), and finally combine it with a time series based rumor classification model. Our extensive experiments show a clearly improved classification performance within the critical very first hours of a rumor. For a better understanding, we also conduct an extensive feature evaluation that emphasized on the early stage and shows that the low-level credibility has best predictability at all phases of the rumor lifetime.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}


==> environs.tex <==
%===================================
%%%%%%%%% Remarks by people
%===================================
\newcommand{\tuan}[1]{{\textcolor{blue}{[\emph{\small Tuan: #1}]}}}
\newcommand{\khoi}[1]{{\textcolor{blue}{[\emph{\small Khoi: #1}]}}}
%\newcommand{\tuan}[1]{{[\emph{\small Tuan: #1}]}}

%===================================
%%%%%%%%% Format
%===================================
\newcommand\vpar{{\vspace*{1em}}}
\newcommand{\para}[1]{\noindent{\textbf{#1.}}}
\newcommand{\parai}[1]{\noindent{\textit{#1.}}}
\newcommand{\term}[1]{{\it {\small #1}}}

\newtheorem{mydef}{Definition}

\newcommand{\superscript}[1]{\ensuremath{^{\textrm{#1}}}}
\def\sharedaffiliation{\end{tabular}\newline\begin{tabular}{c}}
\def\ls{\superscript{1}}
\def\xls{\superscript{1,}}
\def\dfki{\superscript{2}}
\def\dk{\superscript{3}}

%%%%%%%%% Use this when re-formatting \paragraph is absolutely 
%%%%%%%%% necessary, otherwise use Fabian's \para macro
%\renewcommand{\paragraph}[1]{\noindent\textsc{\textsc{#1}}}

%\DeclareMathOperator*{\argmin}{arg\,min}

